2D Wasserstein Loss for Robust Facial Landmark Detection

The recent performance of facial landmark detection has been significantly improved by using deep Convolutional Neural Networks (CNNs), especially the Heatmap Regression Models (HRMs). Although their performance on common benchmark datasets has reached a high level, the robustness of these models still remains a challenging problem in the practical use under noisy conditions of realistic environments. Contrary to most existing work focusing on the design of new models, we argue that improving the robustness requires rethinking many other aspects, including the use of datasets, the format of landmark annotation, the evaluation metric as well as the training and detection algorithm itself. In this paper, we propose a novel method for robust facial landmark detection, using a loss function based on the 2D Wasserstein distance combined with a new landmark coordinate sampling relying on the barycenter of the individual probability distributions. Our method can be plugged-and-play on most state-of-the-art HRMs with neither additional complexity nor structural modifications of the models. Further, with the large performance increase, we found that current evaluation metrics can no longer fully reflect the robustness of these models. Therefore, we propose several improvements to the standard evaluation protocol. Extensive experimental results on both traditional evaluation metrics and our evaluation metrics demonstrate that our approach significantly improves the robustness of state-of-the-art facial landmark detection models.

==> backup.tex <==
\begin{table}[t]
\centering
\begin{tabular}{llll}
\hline
Method & Common & Challenge & Full \\ \hline
PCD-CNN~\cite{kumar2018disentangling} & 3.67 & 7.62 & 4.44 \\
CPM+SBR~\cite{dong2018supervision} & 3.28 & 7.58 & 4.10 \\
SAN~\cite{dong2018san} & 3.34 & 6.60 & 3.98 \\
DAN~\cite{kowalski2017deep} & 3.19 & 5.24 & 3.59 \\
LAB~\cite{wayne2018lab} & 2.98 & \textbf{5.19} & 3.49 \\
DCFE~\cite{valle2018deeply} & \textbf{2.76} & 5.22 & \textbf{3.24} \\ \hline
HRNet, $\sigma=1$, $L2$ & 2.91 & 5.11 & 3.34 \\
$\sigma=3$, $L2$ & 3.05 & 5.28 & 3.49 \\
$\sigma=1$, W Loss & 2.85 & 5.13 & 3.29 \\
$\sigma=3$, W Loss & 3.01 & 5.30 & 3.46 \\
$\sigma=1$, W Loss, CC & \textbf{2.81} & \textbf{5.08} & \textbf{3.26} \\
$\sigma=3$, W Loss, CC & 2.95 & 5.22 & 3.39 \\ \hline
\end{tabular}
\caption{NME (\%) comparison on the300W validation set. W~Loss - Wasserstein Loss. CC - CoordConv.}
\label{Tab:300w_valid_conventional}
\end{table}

On 300W, our model shows comparable performance to the state-of-the-art methods. 
%In terms of ablation study, 
Here, using the Wasserstein loss only achieves a marginal improvement.
And using a larger $\sigma$ even slightly decreases the NME performance. 
As discussed in Sect.~\ref{sec:emp_study}, the performance of vanilla HRNet has already reached a high level on this dataset. Thus, there are only very few challenging validation images for HRNet.
Here, the NME is dominated by a large amount of small errors, which is the disadvantage of using a larger $\sigma$, and it 
%Therefore, the NME on their validation sets 
can thus no longer reflect the robustness of the models. 
We will demonstrate the robustness of these models by using cross-dataset validation in the following experiments.



\begin{figure}[]
\centering
\begin{subfigure}{.4\linewidth}
  \centering
  \includegraphics[width=\textwidth]{Fig/cofw-->aflwall.pdf}
  \caption{COFW$\rightarrow$AFLW-All}
  %\label{fig:sub2}
\end{subfigure}
\begin{subfigure}{.4\linewidth}
  \centering
  \includegraphics[width=\textwidth]{Fig/cofw-->aflwfrontal.pdf}
  \caption{COFW$\rightarrow$AFLW-Frontal}
  %\label{fig:sub2}
\end{subfigure}
\caption{Landmark-wise CED of COFW$\rightarrow$AFLW cross-validation with HRNet.}
\label{fig:cross_cofw}
\end{figure}





